Slicing the stars: counting algebraic numbers, integers, and units by degree and height

Masser and Vaaler have given an asymptotic formula for the number of algebraic numbers of given degree $d$ and increasing height. This problem was solved by counting lattice points (which correspond to minimal polynomials over $\mathbb{Z}$) in a homogeneously expanding star body in $\mathbb{R}^{d+1}$. The volume of this star body was computed by Chern and Vaaler, who also computed the volume of the codimension-one "slice" corresponding to monic polynomials -- this led to results of Barroero on counting algebraic integers. We show how to estimate the volume of higher-codimension slices, which allows us to count units, algebraic integers of given norm, trace, norm and trace, and more. We also refine the lattice point-counting arguments of Chern-Vaaler to obtain explicit error terms with better power savings, which lead to explicit versions of some results of Masser-Vaaler and Barroero.

==> dn.tex <==
[words...]
\begin{theorem}\label{hbound}
The Davenport number $h(\mcU_N)$ does not exceed $(N+1)2^{N-1}.$
%\begin{equation*}
%h(\mcU_N) \leq (N+1)2^{N-2}.
%\end{equation*}
\end{theorem}

Recall that $\mcU_N$ is a compact, symmetric star body in $\RR^{N+1}$.  Let $\ell$ be a line in $\RR^{N+1}$ which is parallel to one of the coordinate axes.  We need an upper bound for the number of connected components of $S_\ell := \ell \cap \mcU_N$.  If $\ell$ passes through the origin, then $S_\ell$ has only one connected component, since $\mcU_N$ is a star-body, so from now on we will assume that $\ell$ does not pass through the origin.  We write $\ell$ parametrically as $(a_0,\dots,t,\dots,a_N), t \in \RR$, having the parameter $t$ in the $i$th coordinate, where the vector $\va = (a_0,\dots,\hat{a_i},\dots,a_N)$ is a nonzero vector in $\RR^N$.

The boundary $\partial \mcU_N$ of $\mcU_N$ described explicitly in \cite[Section 10]{chernvaaler}.  We briefly summarize the key points.  The boundary $\partial \mcU_N$ is the union of $2N+2$ ``patches'' $P_{L,N}^{(\varepsilon)}$, $L = 0,\dots,N$, $\varepsilon = \pm 1$.  The patch $P_{L,N}^{(\varepsilon)}$ is the image of a certain compact set $\mcJ_{L,N}^{(\varepsilon)}$under the map 
\begin{equation}
b_{L,N}^{(\varepsilon)}:\RR^L \times \RR^{N-L} \to \RR^{N+1},
\end{equation}
defined by
\begin{equation}
b_{L,N}^{(\varepsilon)}\big((x_1,\dots,x_L),(y_0,\dots,y_{N-L-1})\big) = B_{L,N}^{(\varepsilon)}\big((1,x_1,\dots,x_L),(y_0,\dots,y_{N-L-1},\varepsilon)\big),
\end{equation}
where the bilinear form $B_{L,N}^{(\varepsilon)}$ is given by
\begin{equation}
B_{L,N}^{(\varepsilon)}\big((x_0,x_1,\dots,x_L),(y_0,\dots,y_{N-L})\big) = (w_0,\dots,w_N),
\end{equation}
with
\begin{equation}
w_n = \sum_{\ell=0}^L \sum_{\shortstack{$m=0$\\$l+m=n$}}^{N-L} x_ly_m, \quad\quad n=0,\dots,N.
\end{equation}

We let $V_{L,N}^{(\varepsilon)}$ denote the full image of $\RR^{L} \times \RR^{N-L}$ under $b_{L,N}^{(\varepsilon)}$, so $V_{L,N}^{(\varepsilon)}$ is a smooth hypersurface in $\RR^{N+1}$ parametrized by two constant or linear functions,
\begin{equation}
w_0 = y_0~\textup{or}~\pm1, \quad w_n = \pm x_L~\textup{or}~\pm 1, 
\end{equation}
and $(N-1)$ quadratic functions $w_1,\dots,w_{N-1}$ in the $N$ variables $x_1,\dots,x_L,y_0,\dots,y_{N-L-1}$.  We'll write $\vx$ for a vector $(x_1,\dots,x_L) \in \RR^L$, and $\vy$ for a vector $(y_0,\dots,y_{N-L-1}) \in \RR^{N-L}$.

%The main part of proving Theorem \ref{hbound} is to establish the following.
%\begin{lemma}\label{onepatchintervals}
%For each $L \in \{0,\dots,N\}$, $\varepsilon \in \{\pm 1\}$, we have that $\ell \cap V_{L,N}^{(\varepsilon)}$ has at most $2^{n-2}$ connected components.
%\end{lemma}
---

STUFF

---

First, we must discuss the number of points in $\ell \cap V_{L,N}^{(\varepsilon)}$.
\begin{lemma}\label{onepatchpoints}
For each $L \in \{0,\dots,N\}$, $\varepsilon \in \{\pm 1\}$, we have that $\ell \cap V_{L,N}^{(\varepsilon)}$, if it is finite, has at most $2^{n-1}$ points.
\end{lemma}
\begin{proof}
The points of intersection of $\ell$ with $V_{L,N}^{(\varepsilon)}$ are in bijection with the set of solutions to the system of equations
\begin{align}
a_n &= w_n(\vx,\vy), \quad \quad n \in \{0,\dots,N\} \setminus \{i\},\label{variety}\\
t &= w_i(\vx,\vy),\label{teq}
\end{align}
in the variables $y, \vx,\vy$.  The system (\ref{variety}) is a system of $N$ polynomial equations in $N$ variables, where at least one of these equations has degree $0$ or $1$, and the rest have degree at most $2$.  Since one equation has degree 0 or 1, this is equivalent to a system of $(N-1)$ polynomial equations in $(N-1)$ variables, each equation having degree at most $2$.  If the solution set is finite, it must have at most $2^{N-1}$ points, according to Bezout's Theorem.  Thus (\ref{variety}) defines an affine variety $X$ in the parameter space $\RR^L\times \RR^{N-L}$, which is the pullback of the line $\ell$ under $b_{L,N}^{(\varepsilon)}$.  As such, the variety $X$ is either a set of at most $2^{n-1}$ points, or else it is a curve (if the system (\ref{variety}) is underdetermined).  Since $w_i$ is linear in each variable separately, we easily see that this ``degenerate'' situation implies that $\ell \cap P_{L,N}^{(\varepsilon)}$ is infinite, and moreover contains at least one line segment of positive length.
If $X$ has finitely many points, notice that the number of points in $\ell \cap V_{L,N}^{(\varepsilon)}$ is no more than the number of points of $X$.  This concludes our proof of the Lemma \ref{onepatchpoints}.
\end{proof}

---

\begin{lemma}\label{budge}
There is a line $\ell'$ parallel $\ell$ such that 
\begin{enumerate}
\item[\textup{(i)}] $\ell' \cap \partial \mcU_N$ is finite, 
\item[\textup{(ii)}] the number of connected components of $S_{\ell'} = \ell' \cap \mcU_N$ is exactly half the number of points in $\ell' \cap \partial \mcU_N$, and
\item[\textup{(iii)}] the number of connected components of $S_{\ell'}$ is the same as that of $S_\ell$.
\end{enumerate}
\end{lemma}
\begin{proof}
[NOTE: The letters $x$ and $y$ in this lemma proof are not related to the $x$'s and $y$'s above.  I haven't decided how to change the notation make this less confusing.  I strongly like keeping the notation above consistent with Chern-Vaaler, but I also strongly like having an ``$x$- and $y$-axis'' below.]
The idea is to move $\ell$ slightly closer to the origin so that it has the desired properties.  Let $W$ denote the plane in $\RR^{N+1}$ containing $\ell$ and the origin, and identify $W$ with $\RR^2$ by taking the origin to be the origin of $\RR^{N+1}$, and taking as a basis unit vectors parallel to (determining the ``$x$-axis'') and perpendicular to (determining the ``$y$-axis'') the line $\ell$.  Let $U = \mcU_N \cap W$, which is a compact, symmetric star-body in $\RR^{2}$.  The boundary $\partial U = W\cap \partial \mcU_N$ is a piecewise-smooth parametrized path, where each path that is not a horizontal line (i.e. a line parallel to $\ell$) has only finitely many critical points.  Let $y_1 = \|\va\|.$  Let $R$ be a closed rectangle in the plane $W$ constructed as follows.
\begin{itemize}
\item The top of $R$ is the line $\ell$, which is given in our coordinates by $y = y_1$.
\item The bottom of $R$ is a parallel line $y=y_0$, with $0< y_0 < y_1$ (it doesn't matter what $y_0$ is).
\item The sides of $R$ are vertical lines $x=x_0$ and $x=x_1$, far enough apart so that $$\{(x,y) \in U ~\big| y_0 \leq y \leq \|\va\|\} \subseteq R.$$
(This is possible because $U$ is compact.)
\end{itemize}
Let $T$ be the closed trapezoid containing $R$, constructed as follows.
\begin{itemize}
\item The bottom of $T$ is the line segment connecting $(x_0,y_0)$ and $(x_1,y_0)$, i.e. the same as the bottom segment of $R$.
\item The sides of $T$ are the passing through $(x_0,y_0)$ and the origin, and the line connecting $(x_1,y_0)$ and the origin.
\item The top of $T$ is the line $y=y_1$, i.e. $\ell$, i.e. a longer segment of the line that forms the top of $R$.
\end{itemize}
 
We now deform $T$ onto $R$ by the following diffeomorphism:
\begin{equation}
\Phi : T \to R, \quad\quad \Phi(x,y) = \left(\frac{xy}{y_0},y\right).
\end{equation}
The map $\Phi$ is simply defined to take the line $\lambda$ passing through the origin to a vertical line $\lambda'$ which intersects $\lambda$ at the point where $y=y_0$, and note that $\Phi$ sends horizontal lines onto themselves.
\begin{figure}
\includegraphics[width=1\textwidth]{Phi.JPG}

A picture of the map $\Phi: T \to R.$

[This is a temporary figure, to be replaced by a better, computer-generated one if this argument makes it into the final version.]
\end{figure}

Observe that, since $U$ is a star-body, $U' := \Phi(U) \cap R$ contains the line segment joining $(x,y)$ with $(x,y_0)$, for every $(x,y) \in U'.$  This amounts to saying that $U$ is the closure of the region below the graph $\Gamma$ of a function.  This graph may contain some vertical or horizontal line segments, but it is a continuous parametric curve, piecewise defined as the images certain curves under the maps $\Phi \circ b_{L,N}^{(\varepsilon)}$.  Because the maps $b$ are just quadratic functions, graph $\Gamma$ has finitely many critical values, i.e $y$-values corresponding to local minima or maxima, or $y$-values of horizontal line segments in $\Gamma$.  This means that there is a line $\ell'$, given in our plane by the equation $y=y_1 - \delta$ for some $\delta > 0$ such that there are no critical values in $[y_1 - \delta,y_1)$.  Even if $y_1$ is a critical value, this means that 
\begin{equation}
\#\pi_0(S_{\ell'}) = \#\pi_0(\ell' \cap U) = \#\pi_0(\ell' \cap U') = \#\pi_0(\ell \cap U') = \#\pi_0(\ell \cap U) = \#\pi_0(S_\ell).
\end{equation}
[Insert whatever we learn from MO??]

Now we have made $\ell'$ so that every intersection point with $\partial U$ (and hence with $\partial U_N$) is a transverse intersection, meaning the line is either ``entering'' or ``exiting'' the set $U$.  There will be an even number of such intersections, and $\pi_0(S_{\ell'}$ consists of exactly one interval for every two intersection points.  This completes our proof of Lemma \ref{budge}.
\end{proof}

\begin{proof}[Proof of Theorem \ref{hbound}]
By Lemma \ref{budge}, the Davenport number of $\mcU_N$ is achieved by a line $\ell'$ satisfying conditions (i)-(iii) of that lemma.  By Lemma \ref{onepatchpoints}, we have
\begin{align*}
h(\mcU_N) &\leq \left(\#\textup{ of patches } P_{L,N}^{(\varepsilon)}\right) \cdot \frac{1}{2}\left(\max_{L,\varepsilon} \# \textup{ of points of} \ell' \cap V_{L,N}^{(\varepsilon)}\right)\\
&\leq (2N+2) \cdot \frac{1}{2}\cdot 2^{N-1} = (N+1)2^{N-1}.
\end{align*}
\end{proof}
[Remark: I think a given line should only be able to touch half of the patches, cutting our bound in half if we can show this.]

%%%%


==> gvheaders.tex <==
\baselineskip=14.5pt

\bibliographystyle{plain}

\makeatletter
\def\imod#1{\allowbreak\mkern10mu({\operator@font mod}\,\,#1)}
\makeatother
\newcommand{\vectornorm}[1]{\left|\left|#1\right|\right|}
\newcommand{\ip}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\ideal}[1]{\left\langle#1\right\rangle}
\newcommand{\sep}[0]{^{\textup{sep}}}
\newcommand{\Span}[0]{\operatorname{Span}}
\newcommand{\Tor}[0]{\operatorname{Tor}}
\newcommand{\Stab}[0]{\operatorname{Stab}}
\newcommand{\Orb}[0]{\operatorname{Orb}}
\newcommand{\Soc}[0]{\operatorname{Soc}}
\newcommand{\Kernel}[0]{\operatorname{ker }}
\newcommand{\Gal}[0]{\operatorname{Gal}}
\newcommand{\Aut}[0]{\operatorname{Aut}}
\newcommand{\Out}[0]{\operatorname{Out}}
\newcommand{\Inn}[0]{\operatorname{Inn}}
\newcommand{\Image}[0]{\operatorname{im }}
\newcommand{\vol}[0]{\operatorname{vol }}
\newcommand{\pgl}[0]{\operatorname{PGL}_2(\mathbb{F}_3)}
\newcommand{\AGL}[0]{\operatorname{AGL}}
\newcommand{\PGL}[0]{\operatorname{PGL}}
\newcommand{\PSL}[0]{\operatorname{PSL}}
\newcommand{\PSp}[0]{\operatorname{PSp}}
\newcommand{\PSU}[0]{\operatorname{PSU}}
\newcommand{\Sp}[0]{\operatorname{Sp}}
\newcommand{\POmega}[0]{\operatorname{P\Omega}}
\newcommand{\Uup}[0]{\operatorname{U}}
\newcommand{\Gup}[0]{\operatorname{G}}
\newcommand{\mcFup}[0]{\operatorname{F}}
\newcommand{\Eup}[0]{\operatorname{E}}
\newcommand{\Bup}[0]{\operatorname{B}}
\newcommand{\Dup}[0]{\operatorname{D}}
\newcommand{\Mup}[0]{\operatorname{M}}
\newcommand{\mini}[0]{\operatorname{min}}
\newcommand{\maxi}[0]{\textup{max}}
\newcommand{\modu}[0]{\textup{mod}}
\newcommand{\nth}[0]{^\textup{th}}
\newcommand{\sd}[0]{\leq_{sd}}
%\newcommand{\deg}[0]{\text{deg }}

 \newtheorem{theorem}{Theorem}[section]
 \renewcommand{\thetheorem}{\arabic{section}.\arabic{theorem}}
 \newtheorem{proposition}[theorem]{Proposition}
   \renewcommand{\theproposition}{\arabic{section}.\arabic{theorem}}
 \newtheorem{lemma}[theorem]{Lemma}
  \renewcommand{\thelemma}{\arabic{section}.\arabic{theorem}}
 \newtheorem{corollary}[theorem]{Corollary}
   \renewcommand{\thecorollary}{\arabic{section}.\arabic{theorem}}
 \newtheorem{conjecture}[theorem]{Conjecture}
   \renewcommand{\theconjecture}{\arabic{section}.\arabic{theorem}}
 \newtheorem{definition}[theorem]{Definition}
   \renewcommand{\thedefinition}{\arabic{section}.\arabic{theorem}}
 \newtheorem{question}[theorem]{Question}
   \renewcommand{\thequestion}{\arabic{section}.\arabic{theorem}}
 \newtheorem*{claim*}{Claim}
 \newtheorem{claim}[theorem]{Claim}
   \renewcommand{\theclaim}{\arabic{section}.\arabic{theorem}}
 \newcommand{\mc}{\mathcal}
 \newcommand{\mf}{\mathfrak}
 \newcommand{\mcA}{\mc{A}}
 \newcommand{\mcB}{\mc{B}}
 \newcommand{\mcC}{\mc{C}}
 \newcommand{\mcD}{\mc{D}}
 \newcommand{\mcE}{\mc{E}}
 \newcommand{\mcF}{\mc{F}}
 \newcommand{\mcG}{\mc{G}}
 \newcommand{\mcH}{\mc{H}}
 \newcommand{\mcI}{\mc{I}}
 \newcommand{\mcJ}{\mc{J}}
 \newcommand{\mcK}{\mc{K}}
 \newcommand{\mcL}{\mc{L}}
 \newcommand{\mcM}{\mc{M}}
 \newcommand{\mcN}{\mc{N}}
 \newcommand{\mcO}{\mc{O}}
 \newcommand{\mcP}{\mc{P}}
 \newcommand{\mcQ}{\mc{Q}}
 \newcommand{\mcR}{\mc{R}}
 \newcommand{\mcS}{\mc{S}} 
 \newcommand{\mcT}{\mc{T}}
 \newcommand{\mcU}{\mc{U}}
 \newcommand{\mcV}{\mc{V}}
 \newcommand{\mcW}{\mc{W}}
 \newcommand{\mcX}{\mc{X}}
 \newcommand{\mcY}{\mc{Y}}
 \newcommand{\mcZ}{\mc{Z}}
 \newcommand{\mfp}{\mf{p}}
 \newcommand{\mfP}{\mf{P}}
 \newcommand{\mfq}{\mf{q}}
 \newcommand{\mfQ}{\mf{Q}}   
 \newcommand{\oQ}{\overline{\QQ}}
 \newcommand{\AAA}{\mathbb{A}}
 \newcommand{\CC}{\mathbb{C}}
 \newcommand{\FF}{\mathbb{F}}
  \newcommand{\GG}{\mathbb{G}}
 \newcommand{\NN}{\mathbb{N}}
 \newcommand{\PP}{\mathbb{P}}
 \newcommand{\QQ}{\mathbb{Q}}
 \newcommand{\QQd}{\QQ^{(d)}}
 \newcommand{\RR}{\mathbb{R}}
 \newcommand{\ZZ}{\mathbb{Z}}
 \newcommand{\oneto}[1]{\{1,\dots,#1\}}
 \newcommand{\tors}[0]{\textup{tors}}
 \newcommand{\QQbar}[0]{\overline{\QQ}}
 \newcommand{\vep}{\varepsilon}
 %Vaaler macros
 \newcommand{\A}[0]{\mcA}
 \newcommand{\B}[0]{\mcB}
 \newcommand{\D}[0]{\mcD}
 \newcommand{\E}[0]{\mcE}
 \newcommand{\F}[0]{\mcF}
 \newcommand{\G}[0]{\mcG} 
 \newcommand{\eL}[0]{\mcL} 
 \newcommand{\M}[0]{\mcM} 
 \newcommand{\X}[0]{\mcX}
 \newcommand{\Q}[0]{\QQ}
 \newcommand{\Z}[0]{\ZZ}
 \newcommand{\zZ}{\mcZ}
 \newcommand{\R}[0]{\RR}
 \newcommand{\spann}[0]{\Span}
 \newcommand{\closure}[0]{\operatorname{closure}}
 \newcommand{\aA}{\mathfrak A}
 \newcommand{\bB}{\mathfrak B}
 \newcommand{\ff}{\mathfrak F}
 \newcommand{\fp}{\mathfrak p}
 \newcommand{\fb}{f_{\beta}}
 \newcommand{\fg}{f_{\gamma}}
 \newcommand{\gb}{g_{\beta}}
 \newcommand{\ep}{\varepsilon}
 \newcommand{\vphi}{\varphi}
 \newcommand{\bo}{\boldsymbol 0}
 \newcommand{\ba}{\boldsymbol a}
 \newcommand{\bb}{\boldsymbol b}
 \newcommand{\bm}{\boldsymbol m}
 \newcommand{\bgamma}{\boldsymbol \gamma}
 \newcommand{\bt}{\boldsymbol t}
 \newcommand{\bu}{\boldsymbol u}
 \newcommand{\bv}{\boldsymbol v}
 \newcommand{\bx}{\boldsymbol x}
 \newcommand{\bwy}{\boldsymbol y}
 \newcommand{\bxi}{\boldsymbol \xi}
 \newcommand{\bbeta}{\boldsymbol \eta}
 \newcommand{\bw}{\boldsymbol w}
 \newcommand{\bz}{\boldsymbol z}
 \newcommand{\whG}{\widehat{G}}
 \newcommand{\oK}{\overline{K}}
 \newcommand{\oKt}{\overline{K}^{\times}}
% \newcommand{\oQ}{\overline{\Q}}
 \newcommand{\oq}{\oQ^{\times}}
 \newcommand{\oQt}{\oQ^{\times}/\Tor\bigl(\oQ^{\times}\bigr)}
 \newcommand{\ot}{\Tor\bigl(\oQ^{\times}\bigr)}
 \newcommand{\h}{\frac12}
 \newcommand{\hh}{\tfrac12}
 \newcommand{\dx}{\text{\rm d}x}
 \newcommand{\dy}{\text{\rm d}y}
 \newcommand{\dmu}{\text{\rm d}\mu}
 \newcommand{\dnu}{\text{\rm d}\nu}
 \newcommand{\dla}{\text{\rm d}\lambda}
 \newcommand{\dlav}{\text{\rm d}\lambda_v}
 \newcommand{\trho}{\widetilde{\rho}}
 \newcommand{\dtrho}{\text{\rm d}\widetilde{\rho}}
 \newcommand{\drho}{\text{\rm d}\rho}
 \newcommand{\wS}{\widetilde{S}}
 \newcommand{\wT}{\widetilde{T}}
   \def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
   {\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}

 \renewcommand{\thefootnote}{\fnsymbol{footnote}}
 % 1   2    3     4     5     6     7     8     9 
 % * \dag                          **
 
 
% \def\today{%\number\time, 
%   \ifcase\month\or
%   January\or February\or March\or April\or May\or June\or
%   July\or August\or September\or October\or November\or December\fi
%   \space\number\day, \number\year}
